How Robustly do LLMs Understand Execution Semantics?

LLMs demonstrate remarkable reasoning capabilities, yet whether they utilize internal world models or rely on sophisticated pattern matching remains open. We study LLMs through the lens of robustness of their code understanding using a standard program-output prediction task. Our results reveal a stark divergence in model behavior: while open-source reasoning models (DeepSeek-R1 family) maintain stable, albeit somewhat lower accuracies (38% to 67%) under code transformations & input perturbations, the frontier model GPT-5.2 exhibits significant brittleness. Despite achieving a near-perfect score of 99% on the original, unperturbed CRUXEval benchmark, perturbed inputs trigger accuracy declines between 20% and 24%. In addition, we find that many models perform much worse at predicting behavior on perturbed inputs that raise exceptions, and that prediction performance depends on the kind of exception. We study remedies to address this deficiency in exception prediction, and evaluate the effect of these remedies on the ability to predict non-exception behaviors. Our findings both point to limitations in the way all models understand code, and establish the value of using perturbation to evaluate code models.

==> includes/biblatex_shim.tex <==
\makeatletter

% 1. Check for the "Both" or "Neither" error states
\@ifpackageloaded{biblatex}{
    \@ifpackageloaded{natbib}{
        % Scenario: BOTH LOADED
        \PackageError{BibliographyShim}{Both biblatex and natbib are loaded, set natbib=false}{Please choose only one bibliography package. This can usually be done by setting natbib=false in the documentclass arguments.}
    }{
        % Scenario: BIBLATEX ONLY (Do nothing, biblatex is native)
    }
}{
    \@ifpackageloaded{natbib}{
        % Scenario: NATBIB ONLY (Apply the shims and warn)
        \PackageWarning{BibliographyShim}{biblatex NOT detected. Applying natbib-to-biblatex shims/aliases for compatibility.}

        % --- Dynamic Filename Capture ---
        \newcommand{\myBibFileName}{main} % Default fallback
        \let\oldbibliography\bibliography
        \renewcommand{\bibliography}[1]{%
            \renewcommand{\myBibFileName}{#1}% Store the name
            \oldbibliography{#1}% Call the original command
        }
        % --------------------------------

        % Aliasing the main commands
        \let\parencite\citep
        \let\textcite\citet
        \let\parencite\citep
        % \let\cite\citep 

        \DeclareRobustCommand{\autocite}{\citep}

        % 2. DISABLE the original natbib commands to force consistency
        \renewcommand{\citet}[2][]{%
            \PackageError{BibliographyShim}{Command \string\citet\space is disabled}{Use \string\textcite\space instead for biblatex compatibility.}%
        }
        \renewcommand{\citep}[2][]{%
            \PackageError{BibliographyShim}{Command \string\citep\space is disabled}{Use \string\parencite\space or \string\autocite\space instead.}%
        }

        % Emulating "Capitalized" commands
        \ifdefined\Citep
            \let\Parencite\Citep
            \let\Textcite\Citet
        \else
            \let\Parencite\citep
            \let\Textcite\citet
        \fi

        % Stubbing out BibLaTeX setup commands 
        \newcommand{\addbibresource}[1]{} 
        
        % The dynamic shim: it uses whatever filename was last stored
        \newcommand{\printbibliography}{\oldbibliography{\myBibFileName}} 

        % (Rest of your previous aliases: \footcite, \citeauthor, etc.)
        % \let\cite\textcite % Or \parencite, depending on your preference
        \let\citeauthor\citeauthor
        \let\citeyear\citeyear
        \newcommand{\footcite}[2][]{\footnote{\citep[#1]{#2}}}

    }{
        % Scenario: NEITHER LOADED
        \PackageError{BibliographyShim}{Neither biblatex nor natbib loaded}{You must load one of these packages for citations to work.}
    }
}

\makeatother

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % BIBLATEX -> NATBIB SHIM
% % Use this to write with modern syntax (\parencite, \textcite) 
% % even when the publisher forces you to use Natbib/BibTeX.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % 1. Aliasing the main commands
% % We use \let to preserve the optional arguments [pg. 2] of natbib
% \let\parencite\citep
% \let\textcite\citet
% % \let\cite\citep % Biblatex \cite is usually parenthetical; adjust if needed

% % 2. Emulating \autocite
% % Change this to \citep or \citet depending on your preference
% \newcommand{\autocite}[2][]{\citep[#1]{#2}}

% % 3. Emulating the "Capitalized" commands
% \let\Parencite\Citep
% \let\Textcite\Citet

% % 4. Emulating specific field commands
% \let\citeauthor\citeauthor
% \let\citeyear\citeyear

% % 5. Handling \footcite (Approximation)
% % Creates a footnote with a parenthetical citation inside
% \newcommand{\footcite}[2][]{\footnote{\citep[#1]{#2}}}

% % 6. Stubbing out BibLaTeX setup commands 
% % (So your code doesn't crash if you leave them in)
% \newcommand{\addbibresource}[1]{} 
% \newcommand{\printbibliography}{\bibliography{references}} % WARNING below

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
